Fair Robust Active Learning by Joint Inconsistency

Fairness and robustness play vital roles in trustworthy machine learning. Observing safety-critical needs in various annotation-expensive vision applications, we introduce a novel learning framework, Fair Robust Active Learning (FRAL), generalizing conventional active learning to fair and adversarial robust scenarios. This framework allows us to achieve standard and robust minimax fairness with limited acquired labels. In FRAL, we then observe existing fairness-aware data selection strategies suffer from either ineffectiveness under severe data imbalance or inefficiency due to huge computations of adversarial training. To address these two problems, we develop a novel Joint INconsistency (JIN) method exploiting prediction inconsistencies between benign and adversarial inputs as well as between standard and robust models. These two inconsistencies can be used to identify potential fairness gains and data imbalance mitigations. Thus, by performing label acquisition with our inconsistency-based ranking metrics, we can alleviate the class imbalance issue and enhance minimax fairness with limited computation. Extensive experiments on diverse datasets and sensitive groups demonstrate that our method obtains the best results in standard and robust fairness under white-box PGD attacks compared with existing active data selection baselines.

==> tables/big_tab.tex <==
\begin{table}[!h]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
\toprule
\multicolumn{7}{c}{UTKFace Four Race Classification (sensitive groups: \{Young, Old\})} \\
\midrule
\multicolumn{1}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard Accuracy (\%)} & \multicolumn{3}{c}{Robust Accuracy (\%)} \\
& Worst ($\uparrow$) & Disp. ($\downarrow$) & Avg. ($\uparrow$)  & Worst ($\uparrow$) & Disp. ($\downarrow$) & Avg. ($\uparrow$) \\

\midrule

Init. AT & 67.58\std{0.30} & 5.38\std{0.25} & 70.27\std{0.31} & 52.98\std{0.08} & 7.26\std{0.31} & 56.61\std{0.06} \\ 

\midrule
    RAND & 70.57\std{0.21} & 4.32\std{0.03} & 72.73\std{0.21} & 55.63\std{0.06} & 7.71\std{0.02} & 59.49\std{0.07} \\
    ENT & 74.10\std{0.79} & 2.45\std{0.48} &  75.33\std{0.56} & 56.94\std{0.64} & 6.60\std{0.33} & 60.25\std{0.56} \\
    CSET & 71.44\std{0.46} & 3.47\std{0.52} & 73.31\std{0.21} & 56.55\std{0.19} & 6.42\std{0.49} & 59.76\std{0.05}  \\
    BADGE & 72.63\std{0.20} & 3.53\std{0.23} & 74.31\std{0.13} & 56.94\std{0.40} & 6.07\std{0.20} & 59.98\std{0.50} \\
    \midrule
    G-RAND & 72.37\std{0.32} & 2.15\std{0.26} & 73.45\std{0.23} & 56.60\std{0.04} & 6.07\std{0.33} & 59.63\std{0.13} \\
    MinMax & 71.35\std{0.24} & 3.27\std{0.28} & 72.98\std{0.20} & 56.95\std{0.22} & 6.59\std{0.12} & 60.25\std{0.21} \\
    OPT &  71.99\std{0.31} & 2.76\std{0.23} & 73.37\std{0.20} & 57.09\std{0.33} & 6.11\std{0.19} & 60.15\std{0.24} \\
    FairAL & 74.74\std{0.31} & 2.20\std{0.13} & \textbf{75.84\std{0.25}} & 56.94\std{0.16} & 6.64\std{0.17} & \textbf{60.47\std{0.07}} \\
    \midrule
    \cellcolor{LightCyan}\textbf{JIN} &  \cellcolor{LightCyan}\textbf{75.07\std{0.53}} & \cellcolor{LightCyan}\textbf{1.35\std{0.09}} & \cellcolor{LightCyan}75.74\std{0.49} & \cellcolor{LightCyan}\textbf{57.39\std{0.10}} & \cellcolor{LightCyan}\textbf{5.69\std{0.30}} & \cellcolor{LightCyan}60.10\std{0.25} \\
    % \midrule
\bottomrule
\end{tabular}
}

\vspace{0.2cm}

\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
\toprule
\multicolumn{7}{c}{CINIC-10 Object Classification (sensitive groups: \{CIFAR-10, ImageNet\})} \\
\midrule
\multicolumn{1}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard Accuracy (\%)} & \multicolumn{3}{c}{Robust Accuracy (\%)} \\
& Worst ($\uparrow$) & Disp. ($\downarrow$) & Avg. ($\uparrow$)  & Worst ($\uparrow$) & Disp. ($\downarrow$) & Avg. ($\uparrow$) \\

\midrule

Init. AT & 52.53\std{0.17} & 12.48\std{0.21} & 58.77\std{0.40} & 31.29\std{0.11} & 10.64\std{0.23} & 36.61\std{0.03} \\ 

\midrule
    RAND & 55.53\std{0.53} & 12.14\std{0.55} & 61.60\std{0.61} & 37.01\std{0.43} & 11.43\std{0.37} & 42.73\std{0.60} \\
    ENT & 56.23\std{0.52} & 11.30\std{0.39} & 61.88\std{0.64} & 36.29\std{0.40} & 10.52\std{0.42} & 41.55\std{0.51} \\
    CSET & 55.28\std{0.44} & 12.94\std{0.51} & 61.75\std{0.52} & 36.73\std{0.27} & 12.22\std{0.52} & \textbf{42.74\std{0.39}} \\
    BADGE & 55.86\std{0.38} & 11.96\std{0.44} & 61.84\std{0.37} & 36.66\std{0.30} & 11.04\std{0.38} & 42.18\std{0.29} \\
    \midrule
    G-RAND & 55.56\std{0.43} & \textbf{10.76\std{0.61}} & 60.94\std{0.66} & 36.71\std{0.35} & 10.02\std{0.41} & 41.72\std{0.59} \\
    MinMax & 55.52\std{0.49} & 11.32\std{0.63} & 61.22\std{0.60} & 36.69\std{0.46} & 10.52\std{0.53} & 41.95\std{0.47} \\
    OPT & 55.78\std{0.33} & 10.90\std{0.37} & 61.23\std{0.49} & 36.90\std{0.29} & ~~9.96\std{0.36} & 41.88\std{0.50} \\
    FairAL & 56.35\std{0.45} & 10.98\std{0.44} & 61.84\std{0.58} & 36.25\std{0.29} & 10.40\std{0.33} & 41.45\std{0.37} \\
    \midrule
    \cellcolor{LightCyan}\textbf{\textbf{JIN}} & \cellcolor{LightCyan}\textbf{57.37\std{0.67}} & \cellcolor{LightCyan}11.16\std{0.52} & \cellcolor{LightCyan}\textbf{62.95\std{0.68}} & \cellcolor{LightCyan}\textbf{37.10\std{0.45}} & \cellcolor{LightCyan}\textbf{~~9.84\std{0.45}} & \cellcolor{LightCyan}42.02\std{0.48} \\
\bottomrule
\end{tabular}
}

\vspace{0.2cm}

\centering
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    \multicolumn{7}{c}{HAM-10000 Skin Lesion Identification (sensitive groups: \{Male, Female\})} \\
    \midrule
    \multicolumn{1}{c|}{
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard F1-score (\%)} & \multicolumn{3}{c}{Robust F1-score (\%)} \\
    & Worst ($\uparrow$) & Disp. ($\downarrow$) & Avg. ($\uparrow$) & Worst ($\uparrow$) & Disp. ($\downarrow$) & Avg. ($\uparrow$)  \\
    
    \midrule
    
    Init. AT &  37.37\std{0.76} & 3.62\std{0.51} & 39.18\std{0.76} & 15.84\std{0.22} & 1.92\std{0.49} & 16.80\std{0.31} \\ 
    
    \midrule
        RAND&40.20\std{0.24}&6.02\std{0.93}&43.21\std{0.58}&19.72\std{0.50}&2.26\std{0.20}&20.85\std{0.44}\\
        ENT&44.34\std{1.14}&6.25\std{0.85}&\textbf{47.46\std{1.54}}&20.11\std{0.51}&3.32\std{0.70}&21.78\std{0.20}\\
        CSET&41.89\std{0.65}&3.70\std{0.88}&43.75\std{0.56}&19.86\std{0.91}& 2.73\std{0.57}&21.22\std{1.19}\\
        BADGE&43.28\std{1.00}&3.52\std{0.46}&45.04\std{0.83}&20.07\std{0.22}&2.39\std{0.39}&21.27\std{0.29}\\
        \midrule
        G-RAND&36.15\std{1.37}&3.46\std{0.61}&37.88\std{1.67}&16.65\std{0.36}&2.85\std{0.89}&18.07\std{0.66}\\
        MinMax&37.21\std{1.21} & 3.59\std{0.86}&39.00\std{1.46}&16.68\std{0.83}&2.17\std{0.80}&17.77\std{0.72}\\
        OPT&35.53\std{1.45}&4.88\std{1.68} & 37.98\std{0.64}&17.32\std{0.38}&\textbf{1.88\std{0.38}}&18.26\std{0.39}\\
        FairAL & 43.65\std{0.99}&3.53\std{0.77}&45.42\std{0.68}&19.64\std{0.54} & 2.44\std{0.81} & 20.86\std{0.83}\\
        \midrule
        \cellcolor{LightCyan}\textbf{JIN}&\cellcolor{LightCyan}\textbf{44.98\std{1.41}}&\cellcolor{LightCyan}\textbf{2.96\std{0.58}} & \cellcolor{LightCyan}46.46\std{1.48}&\cellcolor{LightCyan}\textbf{21.95\std{0.91}}&\cellcolor{LightCyan}2.28\std{0.66}&\cellcolor{LightCyan}\textbf{23.09\std{1.16}}\\
        % \midrule
    \bottomrule
    \end{tabular}
}
    \caption{\textbf{Comparison with various active data selection methods on three diverse datasets with different sensitive attributes.} To ensure the reliability of the experimental results, for each setting, we conduct three experiments with different random seeds and report the average and standard deviation scores. The result demonstrates that our JIN method improves the most standard and robust performance in the worst group on all tasks.}
    
    % Comparison between various active learning methods on the HAM-10000 dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:main_result}
\end{table}

==> tables/cinic10.tex <==
\begin{table*}[!h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc}
\toprule
\multicolumn{8}{c}{CINIC-10 Object Classification (sensitive groups: \{CIFAR-10, ImageNet\})} \\
\midrule
\multicolumn{2}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard Accuracy (\%)} & \multicolumn{3}{c}{Robust Accuracy (\%)} \\
& & Worst ($\uparrow$) & Disparity ($\downarrow$) & Grp. Avg. ($\uparrow$)  & Worst ($\uparrow$) & Disparity ($\downarrow$) & Grp. Avg. ($\uparrow$) \\

\midrule

\multicolumn{2}{c|}{Initialization} & 52.53 \std{0.17} & 12.48 \std{0.21} & 58.77 \std{0.40} & 31.29 \std{0.11} & 10.64 \std{0.23} & 36.61 \std{0.03} \\ 

\midrule
    \multirow{4}*{AL} & 
    RAND & 55.53 \std{0.53} & 12.14 \std{0.55} & 61.60 \std{0.61} & 37.01 \std{0.43} & 11.43 \std{0.37} & 42.73 \std{0.60} \\
    & ENT & 56.23 \std{0.52} & 11.30 \std{0.39} & 61.88 \std{0.64} & 36.29 \std{0.40} & 10.52 \std{0.42} & 41.55 \std{0.51} \\
    & CSET & 55.28 \std{0.44} & 12.94 \std{0.51} & 61.75 \std{0.52} & 36.73 \std{0.27} & 12.22 \std{0.52} & \textbf{42.74 \std{0.39}} \\
    & BADGE & 55.86 \std{0.38} & 11.96 \std{0.44} & 61.84 \std{0.37} & 36.66 \std{0.30} & 11.04 \std{0.38} & 42.18 \std{0.29} \\
    \midrule
    \multirow{4}*{FAL} & G-RAND & 55.56 \std{0.43} & \textbf{10.76 \std{0.61}} & 60.94 \std{0.66} & 36.71 \std{0.35} & 10.02 \std{0.41} & 41.72 \std{0.59} \\
    & MinMax & 55.52 \std{0.49} & 11.32 \std{0.63} & 61.22 \std{0.60} & 36.69 \std{0.46} & 10.52 \std{0.53} & 41.95 \std{0.47} \\
    & OPT & 55.78 \std{0.33} & 10.90 \std{0.37} & 61.23 \std{0.49} & 36.90 \std{0.29} & ~~9.96 \std{0.36} & 41.88 \std{0.50} \\
    & FairAL & 56.35 \std{0.45} & 10.98 \std{0.44} & 61.84 \std{0.58} & 36.25 \std{0.29} & 10.40 \std{0.33} & 41.45 \std{0.37} \\
    \midrule
    \multirow{1}*{\cellcolor{LightCyan}FRAL} 
    % Std-KL & \red{58.22 \std{0.17}} & \red{82.93 \std{0.18}} & 64.21 \std{0.26} & 34.32 \std{0.16} & 76.88 \std{0.03} & 39.48 \std{0.17} \\
    % & Rob-KL & 56.60 \std{0.12} & 81.88 \std{0.19} & 62.86 \std{0.08} & \red{35.23 \std{0.11}} & \red{77.45 \std{0.14}} & 40.46 \std{0.06} \\
    & \cellcolor{LightCyan}\textbf{\textbf{Ours}} & \cellcolor{LightCyan}\textbf{57.37 \std{0.67}} & \cellcolor{LightCyan}11.16 \std{0.52} & \cellcolor{LightCyan}\textbf{62.95 \std{0.68}} & \cellcolor{LightCyan}\textbf{37.10 \std{0.45}} & \cellcolor{LightCyan}\textbf{~~9.84 \std{0.45}} & \cellcolor{LightCyan}42.02 \std{0.48} \\
\bottomrule
\end{tabular}}
    % \caption{Comparison between various active learning methods on the CINIC-10 dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:cinic_result}
    \vspace{-0.5em}
\end{table*}

\iffalse
\begin{table*}[!h]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc}
\toprule
\multicolumn{8}{c}{CINIC-10 Object Classification (sensitive groups: \{CIFAR-10, ImageNet\}) \blue{OLD EXPS}} \\
\midrule
\multicolumn{2}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard Accuracy (\%)} & \multicolumn{3}{c}{Robust Accuracy (\%)} \\
& & Worst ($\uparrow$) & Parity Ratio ($\uparrow$) & Avg.  & Worst ($\uparrow$) & Parity Ratio ($\uparrow$) & Avg.  \\

\midrule

\multicolumn{2}{c|}{Initialization} & 52.53 \std{0.17} & 80.80 \std{0.11} & 58.77 \std{0.40} & 31.29 \std{0.11} & 74.62 \std{0.12} & 36.61 \std{0.03} \\ 

\midrule
    \multirow{4}*{AL} & 
    RAND &  &  & &&& \\
    & ENT & 56.47 \std{0.15} & 81.97 \std{0.11} & 62.68 \std{0.13} & 33.92 \std{0.01} & 75.38 \std{0.03} & 39.46 \std{0.02} \\
    & CSET & 55.28 \std{0.01} & 79.81 \std{0.02} & 62.27 \std{0.02} & 34.64 \std{0.04} & 74.53 \std{0.00} & 40.56 \std{0.05} \\
    & BADGE & 55.93 \std{0.05} & 80.65 \std{0.12} & 62.64 \std{0.11} & & & \\
    \midrule
    \multirow{4}*{FAL} & G-RAND & 55.80 \std{0.14} & 82.00 \std{0.36} & 61.92 \std{0.29} & 34.55 \std{0.07} & 76.45 \std{0.13} & 39.87 \std{0.07} \\
    & FairAL & &&&&& \\
    & MinMax & 1 + dgx1-5  &&&&& \\
    & OPT &  &&& \\
    \midrule
    \multirow{1}*{FRAL} 
    % Std-KL & \red{58.22 \std{0.17}} & \red{82.93 \std{0.18}} & 64.21 \std{0.26} & 34.32 \std{0.16} & 76.88 \std{0.03} & 39.48 \std{0.17} \\
    % & Rob-KL & 56.60 \std{0.12} & 81.88 \std{0.19} & 62.86 \std{0.08} & \red{35.23 \std{0.11}} & \red{77.45 \std{0.14}} & 40.46 \std{0.06} \\
    & \textbf{Ours} & \blue{57.80 \std{0.30}} & \blue{82.29 \std{0.30}} & 64.02 \std{0.46} & \blue{34.78 \std{0.15}} & \blue{77.11 \std{0.36}} & 39.94 \std{0.18} \\
    % \midrule
    % RST &  10.34 \std{1.97} &  86.91 \std{1.83} &  2.40 \std{0.65} &  90.66 \std{0.41} \\
\bottomrule
\end{tabular}}
    \caption{Comparison between various active learning methods on the CINIC-10 dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:cinic_result}
    \vspace{-0.5em}
\end{table*}
\fi 

==> tables/ham.tex <==
\begin{table*}[!h]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccc|ccc}
    \toprule
    \multicolumn{8}{c}{HAM-10000 Skin Lesion Identification (sensitive groups: \{Male, Female\})} \\
    \midrule
    \multicolumn{2}{c|}{
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard F1-score (\%)} & \multicolumn{3}{c}{Robust F1-score (\%)} \\
    & & Worst ($\uparrow$) & Disparity ($\downarrow$) & Grp. Avg. ($\uparrow$) & Worst ($\uparrow$) & Disparity ($\downarrow$) & Grp. Avg. ($\uparrow$)  \\
    
    \midrule
    
    \multicolumn{2}{c|}{Initialization} &  37.37 \std{0.76} & 3.62 \std{0.51} & 39.18 \std{0.76} & 15.84 \std{0.22} & 1.92 \std{0.49} & 16.80 \std{0.31} \\ 
    
    \midrule
        \multirow{4}*{AL} & 
        RAND & 40.20 \std{0.24} & 6.02 \std{0.93} & 43.21 \std{0.58} & 19.72 \std{0.50} & 2.26 \std{0.20} & 20.85 \std{0.44} \\
        & ENT & 44.34 \std{1.14} & 6.25 \std{0.85} & \textbf{47.46 \std{1.54}} & 20.11 \std{0.51} & 3.32 \std{0.70} & 21.78 \std{0.20} \\
        & CSET & 41.89 \std{0.65} & 3.70 \std{0.88} & 43.75 \std{0.56} & 19.86 \std{0.91} & 2.73 \std{0.57} & 21.22 \std{1.19} \\
        & BADGE & 43.28 \std{1.00} & 3.52 \std{0.46} & 45.04 \std{0.83} & 20.07 \std{0.22} & 2.39 \std{0.39} & 21.27 \std{0.29} \\
        \midrule
        \multirow{4}*{FAL} & G-RAND & 36.15 \std{1.37} & 3.46 \std{0.61} & 37.88 \std{1.67} & 16.65 \std{0.36} & 2.85 \std{0.89} & 18.07 \std{0.66} \\
        & MinMax & 37.21 \std{1.21} & 3.59 \std{0.86} & 39.00 \std{1.46} & 16.68 \std{0.83} & 2.17 \std{0.80} & 17.77 \std{0.72} \\
        & OPT & 35.53 \std{1.45} & 4.88 \std{1.68} & 37.98 \std{0.64} & 17.32 \std{0.38} & \textbf{1.88 \std{0.38}} & 18.26 \std{0.39} \\
        & FairAL & 43.65 \std{0.99} & 3.53 \std{0.77} & 45.42 \std{0.68} & 19.64 \std{0.54} & 2.44 \std{0.81} & 20.86 \std{0.83} \\
        \midrule
        \multirow{1}*{\cellcolor{LightCyan}FRAL} 
        & \cellcolor{LightCyan}\textbf{Ours} & \cellcolor{LightCyan}\textbf{44.98 \std{1.41}} & \cellcolor{LightCyan}\textbf{2.96 \std{0.58}} & \cellcolor{LightCyan}46.46 \std{1.48} & \cellcolor{LightCyan}\textbf{21.95 \std{0.91}} & \cellcolor{LightCyan}2.28 \std{0.66} & \cellcolor{LightCyan}\textbf{23.09 \std{1.16}} \\
        % \midrule
    \bottomrule
    \end{tabular}
}
%     \caption{Comparison between various active learning methods on the HAM-10000 dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:ham_result}
    \vspace{-0.5em}
\end{table*}


\iffalse
\begin{table*}[!h]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccc|ccc}
    \toprule
    \multicolumn{8}{c}{HAM-10000 Skin Lesion Identification (sensitive groups: \{Male, Female\})} \\
    \midrule
    \multicolumn{2}{c|}{
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard F1-score (\%)} & \multicolumn{3}{c}{Robust F1-score (\%)} \\
    & & Worst ($\uparrow$) & Pred. Parity ($\downarrow$) & Grp. Avg. ($\uparrow$) & Worst ($\uparrow$) & Pred. Parity ($\downarrow$) & Grp. Avg. ($\uparrow$)  \\
    
    \midrule
    
    \multicolumn{2}{c|}{Initialization} &  37.37 \std{0.76} & 91.30 \std{0.51} & 39.18 \std{0.76} & 15.84 \std{0.22} & 89.96 \std{1.79} & 16.75 \std{0.31} \\ 
    
    \midrule
        \multirow{4}*{AL} & 
        RAND & 40.20 \std{0.24} & 87.23 \std{1.67} & 43.21 \std{0.58} & 19.72 \std{0.50} & 90.39 \std{0.87} & 20.80 \std{0.44} \\
        & ENT & 44.34 \std{1.14} & 87.94 \std{1.38} & \textbf{47.46 \std{1.54}} & 20.11 \std{0.51} & 86.11 \std{2.87} & 21.78 \std{0.20} \\
        & CSET & 41.89 \std{0.65} & 91.96 \std{1.82} & 43.75 \std{0.56} & 19.86 \std{0.91} & 88.35 \std{1.61} & 21.22 \std{1.19} \\
        & BADGE & 43.28 \std{1.00} & 92.61 \std{0.99} & 45.04 \std{0.83} & 20.07 \std{0.22} & 90.61 \std{1.51} & 21.17 \std{0.29} \\
        \midrule
        \multirow{4}*{FAL} & G-RAND & 36.15 \std{1.37} & 93.84 \std{1.27} & 37.38 \std{1.67} & 16.65 \std{0.36} & 85.80 \std{3.77} & 18.07 \std{0.66} \\
        & MinMax & 37.21 \std{1.21} & 91.46 \std{4.08} & 39.00 \std{1.46} & 16.68 \std{0.83} & 88.79 \std{3.72} & 17.77 \std{0.72} \\
        & OPT & 35.53 \std{1.45} & 88.15 \std{3.96} & 37.98 \std{0.64} & 17.32 \std{0.38} & 90.42 \std{1.81} & 18.26 \std{0.39} \\
        & FairAL & 43.65 \std{0.99} & 92.56 \std{2.16} & 45.42 \std{0.68} & 19.64 \std{0.54} & 89.22 \std{3.00} & 20.86 \std{0.83} \\
        \midrule
        \multirow{1}*{\cellcolor{LightCyan}FRAL} 
        & \cellcolor{LightCyan}\textbf{Merge-KL} & \cellcolor{LightCyan}\textbf{44.98 \std{1.41}} & \cellcolor{LightCyan}\textbf{94.02 \std{1.12}} & \cellcolor{LightCyan}46.46 \std{1.48} & \cellcolor{LightCyan}\textbf{21.95 \std{0.91}} & \cellcolor{LightCyan}\textbf{90.75 \std{2.26}} & \cellcolor{LightCyan}\textbf{23.09 \std{1.16}} \\
        % \midrule
    \bottomrule
    \end{tabular}
}
%     \caption{Comparison between various active learning methods on the HAM-10000 dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:ham_result}
    \vspace{-0.5em}
\end{table*}
\fi

==> tables/utkface.tex <==
\begin{table*}[!h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc}
\toprule
\multicolumn{8}{c}{UTKFace 4-Race Classification (sensitive groups: \{Young, Old\})} \\
\midrule
\multicolumn{2}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard Accuracy (\%)} & \multicolumn{3}{c}{Robust Accuracy (\%)} \\
& & Worst ($\uparrow$) & Disparity ($\downarrow$) & Grp. Avg. ($\uparrow$)  & Worst ($\uparrow$) & Disparity ($\downarrow$) & Grp. Avg. ($\uparrow$) \\

\midrule

\multicolumn{2}{c|}{Initialization} & 67.58 \std{0.30} & 5.38 \std{0.25} & 70.27 \std{0.31} & 52.98 \std{0.08} & 7.26 \std{0.31} & 56.61 \std{0.06} \\ 

\midrule
    \multirow{4}*{AL} & 
    RAND & 70.57 \std{0.21} & 4.32 \std{0.03} & 72.73 \std{0.21} & 55.63 \std{0.06} & 7.71 \std{0.02} & 59.49 \std{0.07} \\
    & ENT & 74.10 \std{0.79} & 2.45 \std{0.48} &  75.33 \std{0.56} & 56.94 \std{0.64} & 6.60 \std{0.33} & 60.25 \std{0.56} \\
    & CSET & 71.44 \std{0.46} & 3.47 \std{0.52} & 73.31 \std{0.21} & 56.55 \std{0.19} & 6.42 \std{0.49} & 59.76 \std{0.05}  \\
    & BADGE & 72.63 \std{0.20} & 3.53 \std{0.23} & 74.31 \std{0.13} & 56.94 \std{0.40} & 6.07 \std{0.20} & 59.98 \std{0.50} \\
    \midrule
    \multirow{4}*{FAL} & G-RAND & 72.37 \std{0.32} & 2.15 \std{0.26} & 73.45 \std{0.23} & 56.60 \std{0.04} & 6.07 \std{0.33} & 59.63 \std{0.13} \\
    & MinMax & 71.35 \std{0.24} & 3.27 \std{0.28} & 72.98 \std{0.20} & 56.95 \std{0.22} & 6.59 \std{0.12} & 60.25 \std{0.21} \\
    & OPT &  71.99 \std{0.31} & 2.76 \std{0.23} & 73.37 \std{0.20} & 57.09 \std{0.33} & 6.11 \std{0.19} & 60.15 \std{0.24} \\
    & FairAL & 74.74 \std{0.31} & 2.20 \std{0.13} & \textbf{75.84 \std{0.25}} & 57.14 \std{0.16} & 6.64 \std{0.17} & \textbf{60.47 \std{0.07}} \\
    \midrule
    \multirow{1}*{\cellcolor{LightCyan}FRAL} 
    % Std-KL &  \red{75.77} &  \blue{99.07} &  76.13 & 56.59 & 91.33 & 59.28 (subl*1 + twcc*2)\\
    % & Rob-KL & sublime*2 & twcc &  - & - & - & - \\
    & \cellcolor{LightCyan}\textbf{Ours} &  \cellcolor{LightCyan}\textbf{75.07 \std{0.53}} & \cellcolor{LightCyan}\textbf{1.35 \std{0.09}} & \cellcolor{LightCyan}75.74 \std{0.49} & \cellcolor{LightCyan}\textbf{57.39 \std{0.10}} & \cellcolor{LightCyan}\textbf{5.69 \std{0.30}} & \cellcolor{LightCyan}60.10 \std{0.25} \\
    % \midrule
\bottomrule
\end{tabular}
}
    % \caption{Comparison between various active learning methods on the UTKFace dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:utk_result}
    \vspace{-0.5em}
\end{table*}

\iffalse
\begin{table*}[!h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc}
\toprule
\multicolumn{8}{c}{UTKFace 4-Race Classification (sensitive groups: \{Young, Old\})} \\
\midrule
\multicolumn{2}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods\end{tabular}}} & \multicolumn{3}{c|}{Standard Accuracy (\%)} & \multicolumn{3}{c}{Robust Accuracy (\%)} \\
& & Worst ($\uparrow$) & Parity Ratio ($\uparrow$) & Grp. Avg. ($\uparrow$)  & Worst ($\uparrow$) & Parity Ratio ($\uparrow$) & Grp. Avg. ($\uparrow$) \\

\midrule

\multicolumn{2}{c|}{Initialization} & 67.58 \std{0.30} & 92.58 \std{0.13} & 70.27 \std{0.31} & 52.98 \std{0.08} & 85.09 \std{0.13} & 57.61 \std{0.06} \\ 

\midrule
    \multirow{4}*{AL} & 
    RAND & 70.57 \std{0.21} & 94.22 \std{0.04} & 72.73 \std{0.21} & 55.63 \std{0.06} & 87.83 \std{0.03} & 59.49 \std{0.07} \\
    & ENT & 74.10 \std{0.79} & 96.77 \std{0.66} &  75.33 \std{0.56} & 56.94 \std{0.64} & 89.63 \std{0.52} &  60.25 \std{0.56} \\
    & CSET & 71.44 \std{0.46} & 95.08 \std{0.74} & 73.31 \std{0.21} & 56.55 \std{0.19} & 89.82 \std{0.72} & 59.76 \std{0.05}  \\
    & BADGE & 72.63 \std{0.20} & 95.58 \std{0.30} & 74.31 \std{0.13} & 56.94 \std{0.40} & 90.36 \std{0.22} & 59.98 \std{0.50} \\
    \midrule
    \multirow{4}*{FAL} & G-RAND & 72.37 \std{0.32} & 97.11 \std{0.35} & 73.45 \std{0.23} & 56.60 \std{0.04} & 90.32 \std{0.49} & 59.63 \std{0.13} \\
    & MinMax & 71.35 \std{0.24} & 95.63 \std{0.37} & 72.98 \std{0.20} & 56.95 \std{0.22} & 89.64 \std{0.19} & 60.25 \std{0.21} \\
    & OPT &  71.99 \std{0.31} & 96.31 \std{0.32} & 73.37 \std{0.20} & 57.09 \std{0.33} & 90.34 \std{0.32} & 60.15 \std{0.24} \\
    & FairAL & 74.74 \std{0.31} & 97.13 \std{0.18} & \textbf{75.84 \std{0.25}} & 57.14 \std{0.16} & 89.59 \std{0.27} & \textbf{60.47 \std{0.07}} \\
    \midrule
    \multirow{1}*{\cellcolor{LightCyan}FRAL} 
    % Std-KL &  \red{75.77} &  \blue{99.07} &  76.13 & 56.59 & 91.33 & 59.28 (subl*1 + twcc*2)\\
    % & Rob-KL & sublime*2 & twcc &  - & - & - & - \\
    & \cellcolor{LightCyan}\textbf{Merge-KL} &  \cellcolor{LightCyan}\textbf{75.07 \std{0.53}} & \cellcolor{LightCyan}\textbf{98.24 \std{0.13}} & \cellcolor{LightCyan}75.74 \std{0.49} & \cellcolor{LightCyan}\textbf{57.39 \std{0.10}} & \cellcolor{LightCyan}\textbf{91.40 \std{0.51}} & \cellcolor{LightCyan}60.10 \std{0.25} \\
    % \midrule
\bottomrule
\end{tabular}
}
    % \caption{Comparison between various active learning methods on the UTKFace dataset. The \red{red} and \blue{blue} color indicate the best and the second best result respectively.}
    \label{tab:utk_result}
    \vspace{-0.5em}
\end{table*}

\fi
